Guaranteed Conditional Diffusion: 3D Block-based Models for Scientific Data Compression

This paper proposes a new compression paradigm -- Guaranteed Conditional Diffusion with Tensor Correction (GCDTC) -- for lossy scientific data compression. The framework is based on recent conditional diffusion (CD) generative models, and it consists of a conditional diffusion model, tensor correction, and error guarantee. Our diffusion model is a mixture of 3D conditioning and 2D denoising U-Net. The approach leverages a 3D block-based compressing module to address spatiotemporal correlations in structured scientific data. Then, the reverse diffusion process for 2D spatial data is conditioned on the ``slices'' of content latent variables produced by the compressing module. After training, the denoising decoder reconstructs the data with zero noise and content latent variables, and thus it is entirely deterministic. The reconstructed outputs of the CD model are further post-processed by our tensor correction and error guarantee steps to control and ensure a maximum error distortion, which is an inevitable requirement in lossy scientific data compression. Our experiments involving two datasets generated by climate and chemical combustion simulations show that our framework outperforms standard convolutional autoencoders and yields competitive compression quality with an existing scientific data compression algorithm.

==> Narrative/02RelatedWork_backup.tex <==
\section{Related Work}

\subsection{Diffusion Models}

Diffusion models have emerged as a pivotal class of generative models in machine learning, demonstrating remarkable success across various domains, including image synthesis, natural language processing, and molecular design. This section outlines the foundational works and significant advancements in diffusion models, highlighting key contributions and their impact on the field.

The concept of diffusion models was introduced by Sohl-Dickstein et al.~\cite{Sohl2015}, who proposed a method for deep unsupervised learning using non-equilibrium thermodynamics. This work laid the groundwork for subsequent developments in diffusion-based generative modeling. Building upon this foundation, Song and Ermon~\cite{Song2019} introduced score-based generative modeling, which learns to estimate data gradients and uses them for iterative data generation. This work provided a foundation for noise-agnostic and flexible diffusion processes. Ho et al.~\cite{Ho2020} presented Denoising Diffusion Probabilistic Models (DDPMs), which significantly improved sample quality and training stability. Their approach involved modeling the data distribution through a forward diffusion process and learning to reverse this process to generate new data samples.

Subsequent research has focused on enhancing the efficiency and applicability of diffusion models. Song et al.~\cite{Song2021scorebased} unified diffusion probabilistic models and score-matching approaches through the development of score-based generative models via stochastic differential equations (SDEs). This formulation allowed for a broader understanding and improvement of diffusion processes. Nichol and Dhariwal~\cite{Nichol2021} introduced improved denoising diffusion probabilistic models, addressing limitations in sampling speed and quality. Their work proposed modifications to the noise schedule and model architecture, resulting in faster and more reliable sampling. Dhariwal and Nichol~\cite{Dhariwal2021} demonstrated the competitive performance of diffusion models against state-of-the-art generative adversarial networks (GANs) in high-fidelity image generation tasks. They further introduced classifier guidance for diffusion models to enhance conditional generation. Rombach et al.~\cite{Rombach2022} developed Latent Diffusion Models (LDMs), which operate in a compressed latent space rather than the high-dimensional data space. This approach significantly reduced computational requirements while maintaining high-quality generation, making diffusion models more practical for large-scale applications. More recently, Song et al.~\cite{Song2023} introduced consistency models, which enable efficient one-step sampling by ensuring consistency in generative modeling across forward and reverse processes.

\subsection{Diffusion Models for Compression}
Diffusion models have recently been explored for data compression tasks, leveraging their ability to model complex data distributions. These works demonstrate how diffusion-based generative models can be adapted to achieve state-of-the-art performance in lossy and lossless compression while maintaining high reconstruction quality.

Hoogeboom et al. \cite{Hoogeboom2022autoregressive} introduced Autoregressive Diffusion Models (ARDMs), a model class encompassing and generalizing order-agnostic autoregressive models and absorbing discrete diffusion. ARDMs are simple to implement and easy to train, supporting parallel generation adaptable to any given generation budget. They require significantly fewer steps than discrete diffusion models to attain the same performance and are uniquely suited to lossless compression tasks. 

Yang and Mandt \cite{Yang2023cd} introduced an end-to-end optimized framework for lossy image compression using conditional diffusion models. Their approach relies on the transform coding paradigm, where an image is mapped into a latent space for entropy coding and then reconstructed using a conditional diffusion model. This method introduces an additional ``content'' latent variable to store information about the image, while the remaining ``texture'' variables are synthesized during decoding. The model's performance can be tuned toward perceptual metrics of interest, yielding strong FID scores and competitive distortion metrics. Training the diffusion with $\mathcal{X}$-parameterization enables high-quality reconstructions in only a few decoding steps, enhancing practicality.

Li et al. \cite{Li2024extreme} proposed a novel two-stage extreme image compression framework that exploits the generative capability of pre-trained diffusion models to achieve realistic image reconstruction at extremely low bitrates. The first stage employs a VAE-based compression approach to compress images into content variables, while the second stage leverages pre-trained stable diffusion to reconstruct images under the guidance of these content variables. A small control module injects content information, and a space alignment loss ensures alignment with the diffusion space, providing necessary constraints for optimization. Extensive experiments demonstrate that this method significantly outperforms state-of-the-art approaches in terms of visual performance at extremely low bitrates.

Careil et al. \cite{Careil2024towards} proposed a method for image compression at ultra-low bitrates using iterative diffusion models. Their approach decodes images conditioned on a vector-quantized representation and a global image description, utilizing a two-branch architecture where one branch handles the global structure and the other focuses on local details. This combination allows the model to achieve high-quality reconstructions while preserving important textures and details. The method demonstrates state-of-the-art visual quality as measured by perceptual metrics such as FID and KID, showing that diffusion-based approaches can offer significant advantages over traditional compression techniques.

Relic et al. \cite{Relic2024lossy} formulated the removal of quantization error as a denoising task, using diffusion to recover lost informattted image latent. Their approach allows performing less than 10\% of the full diffusion generative process and requires no architectural changes to the diffusion model, enabling the use of foundation models as a strong prior without additional fine-tuning. The proposed codec outperforms previous methods in quantitative realism metrics, and reconstructions are qualitatively preferred by end users, even when other methods use twice the bitrate.

Ma et al. \cite{ma2024correcting} presented a diffusion-based image compression method that employs a privileged end-to-end decoder model, achieving better perceptual quality while guaranteeing distortion to an extent. They built a diffusion model and designed a novel paradigm combining the diffusion model and an end-to-end decoder, with the latter responsible for transmitting privileged information extracted at the encoder side. Theoretical analysis of the reconstruction process of diffusion models at the encoder side with the original images being visible led to the introduction of an end-to-end convolutional decoder to provide a better approximation of the score function at the encoder side and effectively transmit the combination. Experiments demonstrate the superiority of this method in both distortion and perception compared with previous perceptual compression methods.

These studies collectively highlight the versatility and potential of diffusion models in advancing the field of image compression, offering ns for future research and application.


==> Narrative/02RelatedWork_backup2.tex <==
\section{Related Work}

\subsubsection{Diffusion Models for Image Compression.}

Diffusion models \cite{Sohl2015,Song2019,Ho2020,Song2021scorebased,Nichol2021,Dhariwal2021} have emerged as a dominant class of generative models in machine learning, demonstrating remarkable success across various domains, including image generation and natural language processing. Diffusion models also have recently been explored for image compression tasks. These works demonstrate how diffusion-based generative models can be adapted to achieve state-of-the-art performance in lossy image compression while maintaining high reconstruction quality.

Hoogeboom et al. \cite{Hoogeboom2022autoregressive} introduced Autoregressive Diffusion Models (ARDMs), a model class encompassing and generalizing order-agnostic autoregressive models and absorbing discrete diffusion. ARDMs are simple to implement and easy to train, supporting parallel generation adaptable to any given generation budget. They require significantly fewer steps than discrete diffusion models to attain the same performance and are uniquely suited to lossless compression tasks. 

Yang and Mandt \cite{Yang2023cd} introduced an end-to-end optimized framework for lossy image compression using conditional diffusion models. Their approach relies on the transform coding paradigm, where an image is mapped into a latent space for entropy coding and then reconstructed using a conditional diffusion model. This method introduces an additional ``content'' latent variable to store information about the image, while the remaining ``texture'' variables are synthesized during decoding. The model's performance can be tuned toward perceptual metrics of interest, yielding strong FID scores and competitive distortion metrics. Training the diffusion with $\mathcal{X}$-parameterization enables high-quality reconstructions in only a few decoding steps, enhancing practicality.

Li et al. \cite{Li2024extreme} proposed a novel two-stage extreme image compression framework that exploits the generative capability of pre-trained diffusion models to achieve realistic image reconstruction at extremely low bitrates. The first stage employs a VAE-based compression approach to compress images into content variables, while the second stage leverages pre-trained stable diffusion to reconstruct images under the guidance of these content variables. A small control module injects content information, and a space alignment loss ensures alignment with the diffusion space, providing necessary constraints for optimization. Extensive experiments demonstrate that this method significantly outperforms state-of-the-art approaches in terms of visual performance at extremely low bitrates.

Careil et al. \cite{Careil2024towards} proposed a method for image compression at ultra-low bitrates using iterative diffusion models. Their approach decodes images conditioned on a vector-quantized representation and a global image description, utilizing a two-branch architecture where one branch handles the global structure and the other focuses on local details. This combination allows the model to achieve high-quality reconstructions while preserving important textures and details. The method demonstrates state-of-the-art visual quality as measured by perceptual metrics such as FID and KID, showing that diffusion-based approaches can offer significant advantages over traditional compression techniques.

Relic et al. \cite{Relic2024lossy} formulated the removal of quantization error as a denoising task, using diffusion to recover lost informattted image latent. Their approach allows performing less than 10\% of the full diffusion generative process and requires no architectural changes to the diffusion model, enabling the use of foundation models as a strong prior without additional fine-tuning. The proposed codec outperforms previous methods in quantitative realism metrics, and reconstructions are qualitatively preferred by end users, even when other methods use twice the bitrate.

Ma et al. \cite{ma2024correcting} presented a diffusion-based image compression method that employs a privileged end-to-end decoder model, achieving better perceptual quality while guaranteeing distortion to an extent. They built a diffusion model and designed a novel paradigm combining the diffusion model and an end-to-end decoder, with the latter responsible for transmitting privileged information extracted at the encoder side. Theoretical analysis of the reconstruction process of diffusion models at the encoder side with the original images being visible led to the introduction of an end-to-end convolutional decoder to provide a better approximation of the score function at the encoder side and effectively transmit the combination. Experiments demonstrate the superiority of this method in both distortion and perception compared with previous perceptual compression methods.

Although these studies collectively highlight the versatility and potential of diffusion models for advancing the field of image compression, there is no work that leverages diffusion models in scientific data compression.


==> Narrative/03Methdology_backup.tex <==
\section{Methodology}

We propose a compression pipeline---Guaranteed Conditional Diffusion with Tensor Correction (GCDTC)---for lossy scientific data compression. The framework consists of three steps: (i) conditional diffusion, (ii) tensor correction, and (iii) error guarantee. Our approach leverages conditional generation of diffusion models \cite{Yang2023cd}, where compressed images guide the reverse diffusion process. In our framework, we introduce 3D block conditioning with 2D diffusion models. An overview of our conditional diffusion model is described in Figure~\ref{fig:overview}. Since scientific data have underlying temporal and spatial correlations, they must be addressed for effective data reduction. We first divide the entire dataset into 3D blocks and compress them to get codecs. Then, we use 2D slices of the compressed blocks for conditional generation. There is no advantage in using 3D diffusion models, as spatiotemporal correlations are already addressed by 3D block compression. After the conditional diffusion (CD) model is trained, the reconstructed output of the CD model is further enhanced by a tensor correction network followed by a error guaranteeing process. In this section, we briefly discuss the background of diffusion models and then describe our framework.


\subsection{Background}
%\paragraph{\textbf{Diffusion models}}
\subsubsection{Diffusion models} are a class of hierarchical latent variable models that generate data by iteratively reversing a sequence of noise-adding transformations \cite{Sohl2015,Song2019,Ho2020,Song2021}. These models define a joint distribution over data $\boldsymbol{x}_0$ and latent variables $\boldsymbol{x}_{1:T}$, where the latter represents intermediate noisy versions of the data. The generative process starts from a latent representation drawn from a simple prior (e.g., Gaussian noise) and progressively refines it to produce structured data, such as images.

The forward process $q$ systematically adds noise to the data through a series of Markovian transitions, eroding structure until the data becomes nearly indistinguishable from pure noise:
\begin{equation}\label{eq:forward}
    q\left(\boldsymbol{x}_t|\boldsymbol{x}_{t-1}\right)=\mathcal{N}\left(\boldsymbol{x}_t|\sqrt{1-\beta_t}\boldsymbol{x}_{t-1},\beta_t\boldsymbol{\mathrm{I}}\right),
\end{equation}
where $\beta_t$ is a predefined or learned noise schedule. The reverse process $p_\theta$ uses a neural network to iteratively recover the data by predicting the denoised states:
\begin{equation}\label{eq:reverse}
    p_\theta\left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t,t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}

The reverse process is trained to approximate the true denoising transitions by minimizing a noise-prediction objective. Specifically, the model predicts the added noise $\epsilon$ for a given noisy sample $\boldsymbol{x}_t$, and the loss function is defined as:
\begin{equation}\label{eq:ddpm_loss}
    L\left(\theta,\boldsymbol{x}_0\right)=\mathbb{E}\left\|\epsilon-\epsilon_\theta\left(\boldsymbol{x}_t, t\right)\right\|^2,
\end{equation}
where $\boldsymbol{x}_t$ is constructed as $\boldsymbol{x}_t=\sqrt{\Bar{\alpha}_t}\boldsymbol{x}_0+\sqrt{1-\Bar{\alpha}_t}\epsilon$, $\alpha_t=1-\beta_t$, and $\Bar{\alpha}_t=\prod_{s=1}^t\left(\alpha_s\right)$. By leveraging this objective, the model learns to reverse the forward process and restore data from noise effectively.

For sampling, the reverse process can follow a stochastic trajectory, as in Denoising Diffusion Probabilistic Models (DDPMs) \cite{Ho2020}, or a deterministic path, as in Denoising Diffusion Implicit Models (DDIMs) \cite{Song2021}. The deterministic approach enables faster generation while retaining high-quality results, making it practical for tasks where efficiency is critical.


%\paragraph{\textbf{Conditional diffusion models for compression}}
\subsubsection{Conditional diffusion models for compression}
extend diffusion models to lossy data compression by leveraging conditional generation \cite{Yang2023cd}. In this framework, an image $\boldsymbol{x}_0$ is compressed into a set of latent representations $\boldsymbol{z}$ using an entropy-optimized quantization process. These latent variables are then used as conditioning inputs to guide the reverse diffusion process:
\begin{equation}\label{eq:cd_reverse}
    p_\theta\left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t, \boldsymbol{z}\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t, \boldsymbol{z}, t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
Here, $\boldsymbol{z}$ captures content information about an image, while the reverse diffusion process reconstructs finer texture details progressively. This approach combines the advantages of learned image compression approaches \cite{Balle2017,Balle2018,Minnen2018} with the generative capabilities of diffusion models to propose a new paradigm in lossy image compression. The model is trained using a similar objective to the DDPM loss function in~\eqref{eq:ddpm_loss}, but with an added conditioning mechanism for $\boldsymbol{z}$,
\begin{equation}\label{eq:cd_loss}
    L\left(\boldsymbol{x}_0|\boldsymbol{z}\right)=\mathbb{E}\left\|\epsilon-\epsilon_\theta\left(\boldsymbol{x}_t,\boldsymbol{z}, t\right)\right\|^2=\frac{\Bar{\alpha}_t}{1-\Bar{\alpha}_t}\mathbb{E}\left\|\boldsymbol{x}_0-\mathcal{X}_\theta\left(\boldsymbol{x}_t,\boldsymbol{z}, t\right)\right\|^2,
\end{equation}
where $\mathcal{X}$-prediction, denoted $\mathcal{X}_\theta$, is an equivalent alternative of the noise-based loss function and directly learns to reconstruct $\boldsymbol{x}_0$ instead of the noise $\epsilon$. At test time, the latent variable $\boldsymbol{z}$ is entropy-decoded, and denoising U-Net conditionally reconstructs the image $\boldsymbol{x}_0$ with the iterative reverse process. The sampling process in \cite{Yang2023cd} follows the DDIM's sampling method \cite{Song2021} with either a deterministic way with zero noise or a stochastic noise drawn from a normal distribution. This conditional setup allows the model to work suitably for compression, not generation.


\subsection{3D Conditional Diffusion Model for Scientific Data Compression}

Our approach is developed upon the conditional diffusion model \cite{Yang2023cd}, where latent information $\boldsymbol{z}$ guides the reverse diffusion process for 2D image compression. We extend the conditional diffusion model to 3D scientific data compression, which is a mixture of a 3D block encoder and a conditional 2D denoising U-Net as described in Figure~\ref{fig:cd_model}.
\vspace{-0.4cm}
\subsubsection{Training.}
We first divide the entire dataset into a set of 3D tensors. The tensors are mapped into latent variable $\boldsymbol{z}$ and converted into 3D embedding $\boldsymbol{z}^e$. In the diffusion process, we follow the same method of the DDPM in \eqref{eq:forward} to get the 2D noisy slice $\boldsymbol{x}_{i,t}$ at the stage $t$. Using the slice of the latent embedding $\boldsymbol{z}_i^e$, we modify the conditional reverse diffusion process in \eqref{eq:cd_reverse} as
\begin{equation}\label{eq:our_reverse}
    p_\theta\left(\boldsymbol{x}_{i,t-1}|\boldsymbol{x}_{i,t}, \boldsymbol{z}_i^e\right)=\mathcal{N}\left(\boldsymbol{x}_{i,t-1}|M_\theta\left(\boldsymbol{x}_{i,t}, \boldsymbol{z}_i^e, t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
Like in \eqref{eq:cd_loss}, our model is trained to estimate the noise,
\begin{equation}\label{eq:our_loss}
    L\left(\boldsymbol{x}_{i,0}|\boldsymbol{z}_i^e\right)=\mathbb{E}\left\|\epsilon-\epsilon_\theta\left(\boldsymbol{x}_{i,t},\boldsymbol{z}_i^e, t\right)\right\|^2.
\end{equation}
With the diffusion stage embeddings, the 2D denoising decoder and 3D latent embeddings are trained in an end-to-end manner.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/CD_Model.pdf}
    \caption{A visualization of our 3D conditional diffusion model. We obtain 3D embedding $\boldsymbol{z}^e$ from the tensor block $\boldsymbol{x}$ to effectively address spatiotemporal correlations in scientific datasets. If the tensor block size is $D\times H\times W$, the first dimension of $\boldsymbol{z}^e$ must be equal to $D$. This is because we incorporate 2D diffusion and the $i^\mathrm{th}$ slice $\boldsymbol{z}_i^e$ is used to condition the denoising decoder. Hence, the decoder learns to predict the 2D noise at the diffusion stage $t$ of each 2D slice $\boldsymbol{x}_i$ in $\boldsymbol{x}$. Architecture details are described in Appendix.}\label{fig:cd_model}
    \vspace{-0.4cm}
\end{figure}

%\paragraph{\textbf{Quantization and Decoding.}}

\subsubsection{Quantization and Decoding.}
After the model is trained, we quantize and entropy-encode $\boldsymbol{z}$ using scalar quantization followed by Huffman encoding. Each value $z$ in $\boldsymbol{z}$ is rounded by $\left\lfloor \frac{b}{a}z\right\rfloor$, where $b$ is a power of 10 and $a$ determines the quantization bin size. Then, all the integers are Huffman-encoded to produce compressed codecs. In learned image compression \cite{Balle2017,Balle2018,Minnen2018}, a prior $p\left(\boldsymbol{z}\right)$ is modeled as an additional neural network to include quantization and entropy coding for end-to-end learning. We don't incorporate hyper-prior networks because of (1) additional steps in our framework that complement the output of the CD model and (2) reducing the model complexity.

At decoding time, we entropy-decode and dequantize the compressed codecs and produce latent embeddings. The denoising decoder reconstructs the data deterministically with $\boldsymbol{x}_{i,T}=\boldsymbol{0}$. We reconstruct a 3D tensor $\hat{\boldsymbol{x}}_0$ using ancestral sampling for each 2D slice $\boldsymbol{x}_{i}$ in $\boldsymbol{x}_0$. We follow the DDPM's sampling method,
\begin{equation}
    \boldsymbol{x}_{i,t-1}=\frac{1}{\sqrt{\alpha_t}}\left(\boldsymbol{x}_{i,t}-\frac{1-\alpha_t}{\sqrt{1-\Bar{\alpha}_t}}\epsilon_\theta\left(\boldsymbol{x}_{i,t},\boldsymbol{z}_i^e, t\right)\right).
\end{equation}


\subsection{Tensor Correction and Error Guarantee}\label{subsec:tc_eg}
In lossy scientific data compression, the maximum distortion of reconstructed raw data or primary data (PD) is required to be bounded by a user-specific error target due to reliable post-analysis. For this reason, error-bounded lossy compression is dominant in this field. These techniques are developed upon several methods based on prediction (SZ \cite{SZ3}), transformation (ZFP \cite{ZFP2}), and wavelet decomposition (MGARD \cite{MGARD_3} and SPERR \cite{SPERR}). To provide guaranteed reconstruction, we first enhance the output of the CD model and then correct tensors.
\vspace{-0.6cm}
\subsubsection{Tensor Correction.}
We incorporate a tensor correction (TC) network proposed in \cite{JL-S3D_arxiv}. The TC network is trained using reconstructed tensors obtained from the CD model, and it is an ``overcomplete'' feedforward network to learn a reverse mapping from the reconstructed tensor $\hat{\boldsymbol{x}}$ to the original tensor $\boldsymbol{x}$. In our TC network, we use tensors along the perpendicular direction to 2D slices in the CD model. The TC network reproduces the enhanced reconstructed dataset $\hat{X}$.
%\paragraph{\textbf{Error Guarantee.}}
\subsubsection{Error Guarantee.}
We utilize a post-processing method to control a maximum error distortion according to a pre-specified error bound \cite{JL-GAE,JL-S3D_arxiv}. We first divide the original and reconstructed datasets into small blocks ($\{\boldsymbol{b}\}_{i=1}^N$ and $\{\hat{\boldsymbol{b}}\}_{i=1}^N$) to bound errors on this small region. We perform PCA on the residual set $\{\boldsymbol{b}-\hat{\boldsymbol{b}}\}_{i=1}^N$ to get a global basis $U$. The error guarantee step is a selective process. For each block $\boldsymbol{b}$ that exceeds the error bound $\tau$ ($\|\boldsymbol{b}-\hat{\boldsymbol{b}}\|_{2}> \tau$), we draw coefficients by projecting its residual onto the subspace spanned by the basis $U$,
\begin{equation}
    \boldsymbol{c}=U^T\left(\boldsymbol{b}-\hat{\boldsymbol{b}}\right).
\end{equation}
The coefficient $\boldsymbol{c}$ is quantized using log-based scalar quantization \cite{JL-S3D_arxiv}. We dequantize the coefficient and sort its entries according to their contribution to the $\ell_2$ error of $\hat{\boldsymbol{b}}$. We select the optimal subset $\boldsymbol{c}_s$ in $\boldsymbol{c}$ and its corresponding basis set $U_s$ to satisfy the target error bound. The final corrected block $\Tilde{\boldsymbol{b}}$ is
\begin{equation}
    \Tilde{\boldsymbol{b}}=\hat{\boldsymbol{b}}+U_{s}\boldsymbol{c}_{s}.
\end{equation}
The selected coefficients and basis indices are encoded using Huffman encoding. In our framework, the compressed codecs include all the encoded data of latent variables in the CD model and selected coefficients with their indices. We also consider all the models, PCA basis, and dictionaries of entropy coding for compression costs. Otherwise, we can use an extremely large machine that is even larger than the given scientific dataset, and can do overfitting to produce ideal results. This is because scientific datasets are domain-specific, unlike natural image compression.

==> Narrative/Backup.tex <==
\section{Methodology}

\subsection{Background}
\paragraph{\textbf{Denoising diffusion models}} are hierarchical latent variable models that generate data by a sequence of iterative stochastic denoising steps \cite{Sohl2015,Yang2019,Ho2020,Song2021}. These models describe a joint distribution over data $\boldsymbol{x}_0$ and latent variables $\boldsymbol{x}_{1:T}$ such that $p_\theta\left(\boldsymbol{x}_0\right)=\int p_\theta\left(\boldsymbol{x}_{1:T}\right)d\boldsymbol{x}_{1:T}$. While a diffusion process (denoted by $q$)  incrementally \textit{destroys} structure, its reverse process $p_\theta$ \textit{generates} structure. Both processes involve Markovian dynamics between a sequence of transitional steps (denoted by $t$), where
\begin{equation}\label{eq:forward}
    q\left(\boldsymbol{x}_t|\boldsymbol{x}_{t-1}\right)=\mathcal{N}\left(\boldsymbol{x}_t|\sqrt{1-\beta_t}\boldsymbol{x}_{t-1},\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
\begin{equation}\label{eq:reverse}
    p_\theta\left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t,t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
The variance schedule $\beta\in \left(0,1\right)$ can be either fixed or learned; besides it, the diffusion process is parameter-free. The denoising process predicts the posterior mean from the diffusion process and is parameterized by a neural network $M_\theta\left(\boldsymbol{x}_t,t\right)$.

Denoising Diffusion Probabilistic Model (DDPM) \cite{Ho2020} showed a tractable objective function for training the reverse process. A simplified version of their objective resulted in the following \textit{noise parameterization}, where one seeks to predict the noise $\epsilon$ used to perturb a particular image $\boldsymbol{x}_0$ from the noisy image $\boldsymbol{x}_t$ at noise level $t$:
\begin{equation}
    L\left(\theta,\boldsymbol{x}_0\right)=\mathbb{E}\left\|\epsilon-\epsilon_\theta\left(\boldsymbol{x}_t\left(\boldsymbol{x}_0\right)\right),t\right\|^2.
\end{equation}
Above, $t\sim\textrm{unif}\{1,T\}$, $\epsilon\sim \mathcal{N}\left(\boldsymbol{0},\boldsymbol{\mathrm{I}}\right)$, $\boldsymbol{x}_t\left(\boldsymbol{x}_0\right)=\sqrt{\alpha_t}\boldsymbol{x}+\sqrt{1-\alpha_t}\epsilon$, and $\alpha_t=\prod_{i=1}^t\left(1-\beta_i\right)$. At test time, data can be generated by ancestral sampling using Langevin dynamics. Alternatively, \cite{Song2021} proposed the Denoising Diffusion Implicit Model (DDIM) that follows a deterministic generation procedure after an initial stochastic draw from the prior. Our paper uses the DDIM scheme at test time.

\paragraph{\textbf{Diffusion models}} are hierarchical latent variable models that iteratively generate data through a sequence of stochastic denoising steps \cite{Sohl2015,Yang2019,Ho2020,Song2021}. These models define a joint distribution over the observed data $\boldsymbol{x}_0$ and a sequence of latent variables $\boldsymbol{x}_{1:T}$ such that $p_\theta\left(\boldsymbol{x}_0\right)=\int p_\theta\left(\boldsymbol{x}_{1:T}\right)d\boldsymbol{x}_{1:T}$. The generative process relies on reversing a forward diffusion process $q$, which progressively adds noise to the data until it becomes indistinguishable from Gaussian noise. This forward process is described by Markov transitions:
\begin{equation}\label{eq:forward}
    q\left(\boldsymbol{x}_t|\boldsymbol{x}_{t-1}\right)=\mathcal{N}\left(\boldsymbol{x}_t|\sqrt{1-\beta_t}\boldsymbol{x}_{t-1},\beta_t\boldsymbol{\mathrm{I}}\right),
\end{equation}
where $\beta_t$ is a variance schedule that can be either fixed or learned. The reverse process $p_\theta$ reconstructs structure from noise using a parameterized neural network:
\begin{equation}\label{eq:reverse}
    p_\theta\left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t,t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
Here, $M_\theta\left(\boldsymbol{x}_t,t\right)$ predicts the posterior mean of the reverse process at each time step $t$.

The objective for training the reverse process is derived from a simplified variational lower bound \cite{Ho2020}, leading to the noise prediction formulation. The loss function minimizes the difference between the true noise $\epsilon$ and the predicted noise $\epsilon_\theta$:
\begin{equation}
    L\left(\theta,\boldsymbol{x}_0\right)=\mathbb{E}\left\|\epsilon-\epsilon_\theta\left(\boldsymbol{x}_t\left(\boldsymbol{x}_0\right),t\right)\right\|^2,
\end{equation}
where $\boldsymbol{x}_t$ is computed as $\boldsymbol{x}_t\left(\boldsymbol{x}_0\right)=\sqrt{\alpha_t}\boldsymbol{x}_0+\sqrt{1-\alpha_t}\epsilon$, $\alpha_t=\prod_{i=1}^t\left(1-\beta_i\right)$, and $\epsilon\sim \mathcal{N}\left(\boldsymbol{0},\boldsymbol{\mathrm{I}}\right)$. During generation, data is synthesized through ancestral sampling or deterministic procedures such as DDIM \cite{Song2021}, which enhances sampling efficiency.

\paragraph{\textbf{Conditional diffusion models}} incorporate diffusion models for compression. The basis of our compression approach is a new latent variable model: the diffusion variational autoencoder. This model has a ``semantic'' latent variable $\boldsymbol{z}$ for encoding the image content, and a set of ``texture'' variables $\boldsymbol{x}_{1:T}$ describing residual information,
\begin{equation}
    p\left(\boldsymbol{x}_{0:T},\boldsymbol{z}\right)=p\left(\boldsymbol{x}_{0:T}|\boldsymbol{z}\right)p\left(\boldsymbol{z}\right).
\end{equation}
As detailed below, the decoder will follow a denoising process conditioned on $\boldsymbol{z}$ Drawing on methods
 described in Section 3.1, we use a neural encoder $e\left(\boldsymbol{z}|\boldsymbol{x}_{0}\right)$ to encode the image. The prior $p\left(\boldsymbol{z}\right)$  is a
 two-level hierarchical prior (commonly used in learned image compression) and is used for entropy coding $\boldsymbol{z}$ after quantization. Next, we discuss the novel decoder model.

\paragraph{\textbf{ Decoder and training objective}} We construct the conditional denoising diffusion model in a similar way to the non-variational diffusion autoencoder of \cite{Preechakul2021,Wang2023info}. In analogy to Eq. \eqref{eq:forward,eq:reverse}, we introduce a conditional denoising diffusion process for decoding the latent $\boldsymbol{z}$,
\begin{equation}
    p_\theta\left(\boldsymbol{x}_{0:T}|\boldsymbol{z}\right)=p\left(\boldsymbol{x}_T\right)\prod p_{\theta} \left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_{t},\boldsymbol{z}\right)=p\left(\boldsymbol{x}_T\right)\prod \mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t,\boldsymbol{z},t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
Since the texture latent variables $\boldsymbol{x}_{1:T}$ are not compressed but synthesized at decoding time, the optimal encoder and prior should be learned jointly with the decoder’s marginal likelihood. $p\left(\boldsymbol{x}_{0}|\boldsymbol{z}\right)=\int p\left(\boldsymbol{x}_{0:T}|\boldsymbol{z}\right)d\boldsymbol{x}_{1:T}$ while targeting a certain tradeoff between rate and distortion specified by a Lagrange parameter $\lambda$. We can upper-bound this rate-distortion (R-D) objective by invoking Jensen’s inequality,

\paragraph{\textbf{Conditional diffusion models for compression}} extend diffusion models to lossy data compression by leveraging conditional generation \cite{Yang2023cd}. In this framework, an image $\boldsymbol{x}_0$ is compressed into a set of latent representations $\boldsymbol{z}$ using an entropy-optimized quantization process. These latent variables are then used as conditioning inputs to guide the reverse diffusion process:
\begin{equation}
    p_\theta\left(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t, \boldsymbol{z}\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1}|M_\theta\left(\boldsymbol{x}_t, \boldsymbol{z}, t\right),\beta_t\boldsymbol{\mathrm{I}}\right).
\end{equation}
Here, $\boldsymbol{z}$ captures global information about the image, while the reverse diffusion process reconstructs finer details progressively. This approach combines the advantages of traditional entropy coding with the generative capabilities of diffusion models to achieve high-quality reconstruction at low bitrates.

The model is trained using a similar objective to standard diffusion models, but with an added conditioning mechanism for $\boldsymbol{z}$. At test time, the forward diffusion process maps decoded latents back to a noisy representation, from which the reverse process iteratively reconstructs the original image. This conditional setup allows the model to balance reconstruction quality and perceptual realism, adapting to different compression needs.


\subsection{3D Conditional Diffusion Model for Scientific Data Compression}

\subsection{Error Guarantees}
